Multiview Contextual Commonsense Inference: A New Dataset and Task

Contextual commonsense inference is the task of generating various types of explanations around the events in a dyadic dialogue, including cause, motivation, emotional reaction, and others. Producing a coherent and non-trivial explanation requires awareness of the dialogue's structure and of how an event is grounded in the context. In this work, we create CICEROv2, a dataset consisting of 8,351 instances from 2,379 dialogues, containing multiple human-written answers for each contextual commonsense inference question, representing a type of explanation on cause, subsequent event, motivation, and emotional reaction. We show that the inferences in CICEROv2 are more semantically diverse than other contextual commonsense inference datasets. To solve the inference task, we propose a collection of pre-training objectives, including concept denoising and utterance sorting to prepare a pre-trained model for the downstream contextual commonsense inference task. Our results show that the proposed pre-training objectives are effective at adapting the pre-trained T5-Large model for the contextual commonsense inference task.

==> rebuttal.tex <==
% https://docs.google.com/document/d/1QozfluEiQxOF0Y1wwMxYbD_2aH5KQNuT3mtjUIqc1d4/edit
Review #1
Weaknesses:

1.    There is a large degree of overlap between this study and previous CICEROv1 work.

2.    It's better to show the recall results in Tables 3, 4, and 5.

3.    Experimental results in Tables 4 and 5 didn't show which pre-training tasks contribute to the performance gain. How about using each objective at a time?

Reasons to reject
This CICEROv2 paper is an extension of the previous CICERO paper and there is a large percentage of overlap, e.g., the construction part, and pre-training objectives in Section 4.2, Figures 1, 2, and Tables 1, 7.



Review #2
Main Weaknesses:

1) in a technical sense, the paper is difficult to follow. There are no examples showing a) how CICERO is limited with respect to the multi-view perspective proposed, b) how CICEROv2 improves with respect to CICERO

2) there is no theoretical motivation for the idea of the multi-view perspective of the explanations. This idea is interesting, but it seems to be based on common sense. There are no citations about how, why this idea may advance this type of dataset. Thus, it is unclear to me why a multi-view perspective dataset (CICEROv2) will be better than a dataset where the explanations are semantically similar (CICERO). In my view, the former dataset doesn't necessarily means better in any sense, just different, while the latter dataset may be seen as a challenging dataset due to the lexical overlap and semantic similarity of the explanations (provided that the instances are well-annotated in both datasets)

3) I have a concern about a dimension not taken into account in CICEROv2. According to the authors, CICEROv2 does not include the 'Prerequisite' dimension from CICERO since annotators confused it with the 'Cause' dimension. I wonder how could the annotators in CICERO distinguish from these two dimensions? There doesn't seem to be any attempt to clarify this issue in this paper and thus this dimension is not included. I'm not sure to what extent this dimension is actually useful or necessary to be included in the dataset.

4) Some of the annotation examples provided are confusing to me. For example, for the target utterance in Figure 2, considering the direct-cause event, the first generated correct answer seems to somehow contradict the dialogue since the speaker said "At first I was going to use the oranges, but I think these will taste better" (the speaker is referring to bananas); the generated answer was "It is too difficult to process the orange pulp"; however, the speaker is saying that the reason for using bananas instead of oranges is the taste. So, I would expect a direct-cause such as "I like more bananas because they are sweeter than oranges". Also, from Figure 2, in the case of an emotional-reaction event, the first incorrect answer generated is confusing to me since it is not contradicting the correct answer, it is very similar answer just with different words. Overall, I'm not sure to what extent my expectations holds true; the way how the annotation scheme is framed is confusing to me.

5) In Section 3.2, the sampling of dialogues and targets for CICEROvs is described but there is no rationale of why it is like this.

6) I find a little bit odd that the model used, T5, is pretrained on CICERO rather than on CICEROv2. If the authors made the claim about CICERO not capturing the multi-view perspective, and then they claim to have fixed this issue, then why bother using CICERO?

7) As shown in Table 3, the F1-score gains between T5 and DIALECT (T5 after pretraining with the proposed loss objectives) are not that substantial. It seems like a lot of pre-training effort to get this improvement in scores.

8) There is a finding that the authors seem to be missing from Table 6; in average, when CICEROv2 is tested on CICERO it gets 0.2694 points, and when CICERO is tested on CICEROv2 it gets 0.3321 points in average. This seems to show that CICERO can manage to do better on CICEROv2's test set than the other way around.

Reasons to reject
1) The paper is a bit difficult to follow.
2) The motivation for augmenting CICERO is not well supported by neither theory nor examples

3) The results shown focus more on how good are the pretraining objectives proposed rather than what can we gain from CICEROv2 with respect to CICERO. I consider important that the authors had tested this difference, probably through error analysis, to see if there is any systematic trend of improvement, specially testing their idea of the multi-view perspective.


Review #3


==> table/input_output_example.tex <==
1a

What is or could be the cause of target? \n target: Just one, Mr. Blank. You had a telephone call from someone called Brown, David Brown. \n context: A: Any messages, Miss Grey? <utt> B: Just one, Mr. Blank. You had a telephone call from someone called Brown, David Brown. <utt> A: Brown? I don't seem to know anyone called Brown. What did he say? <utt> B: He wouldn't say. But it sounded important. I told him you'd phone him as soon as you got back. <utt> A: Well, I'd better do it then, I suppose. Er...you've got his phone number, haven't you? <utt> B: Yes, it's 633201. <utt> A: 622301. <utt> B: No, 633201. <utt> A: Oh, I'd better write it down, otherwise I'll probably forget it. <utt> B: I have already done it, Mr. Blank. It's on your desk.

Miss grey received a phone call from david brown when mr blank was not in his office.

1b

For which utterance in the context the cause is the following: Miss grey received a phone call from david brown when mr blank was not in his office. \n context: A: Any messages, Miss Grey? <utt> B: Just one, Mr. Blank. You had a telephone call from someone called Brown, David Brown. <utt> A: Brown? I don't seem to know anyone called Brown. What did he say? <utt> B: He wouldn't say. But it sounded important. I told him you'd phone him as soon as you got back. <utt> A: Well, I'd better do it then, I suppose. Er...you've got his phone number, haven't you? <utt> B: Yes, it's 633201. <utt> A: 622301. <utt> B: No, 633201. <utt> A: Oh, I'd better write it down, otherwise I'll probably forget it. <utt> B: I have already done it, Mr. Blank. It's on your desk.

Just one, Mr. Blank. You had a telephone call from someone called Brown, David Brown.

2a

For which utterance in the context the cause is related to the following concepts: receive, phone, blank, office \n context: A: Any messages, Miss Grey? <utt> B: Just one, Mr. Blank. You had a telephone call from someone called Brown, David Brown. <utt> A: Brown? I don't seem to know anyone called Brown. What did he say? <utt> B: He wouldn't say. But it sounded important. I told him you'd phone him as soon as you got back. <utt> A: Well, I'd better do it then, I suppose. Er...you've got his phone number, haven't you? <utt> B: Yes, it's 633201. <utt> A: 622301. <utt> B: No, 633201. <utt> A: Oh, I'd better write it down, otherwise I'll probably forget it. <utt> B: I have already done it, Mr. Blank. It's on your desk.

Just one, Mr. Blank. You had a telephone call from someone called Brown, David Brown.

2b

For which utterance in the context the cause is the following: Miss grey received a phone call from david brown when mr blank was not in his office. \n concept: telephone \n context: A: Any messages, Miss Grey? <utt> B: Just one, Mr. Blank. You had a telephone call from someone called Brown, David Brown. <utt> A: Brown? I don't seem to know anyone called Brown. What did he say? <utt> B: He wouldn't say. But it sounded important. I told him you'd phone him as soon as you got back. <utt> A: Well, I'd better do it then, I suppose. Er...you've got his phone number, haven't you? <utt> B: Yes, it's 633201. <utt> A: 622301. <utt> B: No, 633201. <utt> A: Oh, I'd better write it down, otherwise I'll probably forget it. <utt> B: I have already done it, Mr. Blank. It's on your desk.

Just one, Mr. Blank. You had a telephone call from someone called Brown, David Brown.

3a

What is or could be the cause of target? \n concepts in the target: telephone \n context: A: Any messages, Miss Grey? <utt> B: Just one, Mr. Blank. You had a telephone call from someone called Brown, David Brown. <utt> A: Brown? I don't seem to know anyone called Brown. What did he say? <utt> B: He wouldn't say. But it sounded important. I told him you'd phone him as soon as you got back. <utt> A: Well, I'd better do it then, I suppose. Er...you've got his phone number, haven't you? <utt> B: Yes, it's 633201. <utt> A: 622301. <utt> B: No, 633201. <utt> A: Oh, I'd better write it down, otherwise I'll probably forget it. <utt> B: I have already done it, Mr. Blank. It's on your desk.

Miss grey received a phone call from david brown when mr blank was not in his office.

3b

What is or could be the cause of target? \n target: Just one, Mr. Blank. You had a telephone call from someone called Brown, David Brown. \n concepts in the answer: receive, phone, blank, office \n context: A: Any messages, Miss Grey? <utt> B: Just one, Mr. Blank. You had a telephone call from someone called Brown, David Brown. <utt> A: Brown? I don't seem to know anyone called Brown. What did he say? <utt> B: He wouldn't say. But it sounded important. I told him you'd phone him as soon as you got back. <utt> A: Well, I'd better do it then, I suppose. Er...you've got his phone number, haven't you? <utt> B: Yes, it's 633201. <utt> A: 622301. <utt> B: No, 633201. <utt> A: Oh, I'd better write it down, otherwise I'll probably forget it. <utt> B: I have already done it, Mr. Blank. It's on your desk.

Miss grey received a phone call from david brown when mr blank was not in his office.

4

What is or could be the cause of target? \n target: Just one, Mr. Blank. You had a telephone call from someone called Brown, David Brown. \n (0) Miss grey received a phone call from david brown while mr blank was at work.(1) Miss grey received a phone call from mr blank when mr blank was in his office.(2) Miss grey received a phone call form david brown while mr blank was already home.(3) Mr blank received a phone call from david brown.(4) Miss grey received a phone call from david brown when mr blank was not in his office. \n context: A: Any messages, Miss Grey? <utt> B: Just one, Mr. Blank. You had a telephone call from someone called Brown, David Brown. <utt> A: Brown? I don't seem to know anyone called Brown. What did he say? <utt> B: He wouldn't say. But it sounded important. I told him you'd phone him as soon as you got back. <utt> A: Well, I'd better do it then, I suppose. Er...you've got his phone number, haven't you? <utt> B: Yes, it's 633201. <utt> A: 622301. <utt> B: No, 633201. <utt> A: Oh, I'd better write it down, otherwise I'll probably forget it. <utt> B: I have already done it, Mr. Blank. It's on your desk.

Miss grey received a phone call from david brown when mr blank was not in his office.

5

answer: Miss grey received a phone call from david brown when mr blank was not in his office. \n target: Just one, Mr. Blank. You had a telephone call from someone called Brown, David Brown. \n context: A: Any messages, Miss Grey? <utt> B: Just one, Mr. Blank. You had a telephone call from someone called Brown, David Brown. <utt> A: Brown? I don't seem to know anyone called Brown. What did he say? <utt> B: He wouldn't say. But it sounded important. I told him you'd phone him as soon as you got back. <utt> A: Well, I'd better do it then, I suppose. Er...you've got his phone number, haven't you? <utt> B: Yes, it's 633201. <utt> A: 622301. <utt> B: No, 633201. <utt> A: Oh, I'd better write it down, otherwise I'll probably forget it. <utt> B: I have already done it, Mr. Blank. It's on your desk.

cause

6

The cause of the target: Miss grey received a phone call from david brown when mr blank was not in his office. \n target options: Just one, Mr. Blank. You had a telephone call from someone called Brown, David Brown. <utt> He wouldn't say. But it sounded important. I told him you'd phone him as soon as you got back. <utt> 622301. <utt> Any messages, Miss Grey? \n context: A: Any messages, Miss Grey? <utt> B: Just one, Mr. Blank. You had a telephone call from someone called Brown, David Brown. <utt> A: Brown? I don't seem to know anyone called Brown. What did he say? <utt> B: He wouldn't say. But it sounded important. I told him you'd phone him as soon as you got back. <utt> A: Well, I'd better do it then, I suppose. Er...you've got his phone number, haven't you? <utt> B: Yes, it's 633201. <utt> A: 622301. <utt> B: No, 633201. <utt> A: Oh, I'd better write it down, otherwise I'll probably forget it. <utt> B: I have already done it, Mr. Blank. It's on your desk.

Just one, Mr. Blank. You had a telephone call from someone called Brown, David Brown.

7

target: Just one, Mr. Blank. You had a telephone call from someone called Brown, David Brown. \n The cause of the target: Miss grey received a phone call from david brown when mr blank was not in his office. \n What is the subsequent event of the target? \n context: A: Any messages, Miss Grey? <utt> B: Just one, Mr. Blank. You had a telephone call from someone called Brown, David Brown. <utt> A: Brown? I don't seem to know anyone called Brown. What did he say? <utt> B: He wouldn't say. But it sounded important. I told him you'd phone him as soon as you got back. <utt> A: Well, I'd better do it then, I suppose. Er...you've got his phone number, haven't you? <utt> B: Yes, it's 633201. <utt> A: 622301. <utt> B: No, 633201. <utt> A: Oh, I'd better write it down, otherwise I'll probably forget it. <utt> B: I have already done it, Mr. Blank. It's on your desk.

The listener tries to recall if he knows mr. brown personally.

8

target: Just one, Mr. Blank. You had a telephone call from someone called Brown, David Brown. \n corrupted concepts: blank, phone, office \n context: A: Any messages, Miss Grey? <utt> B: Just one, Mr. Blank. You had a telephone call from someone called Brown, David Brown. <utt> A: Brown? I don't seem to know anyone called Brown. What did he say? <utt> B: He wouldn't say. But it sounded important. I told him you'd phone him as soon as you got back. <utt> A: Well, I'd better do it then, I suppose. Er...you've got his phone number, haven't you? <utt> B: Yes, it's 633201. <utt> A: 622301. <utt> B: No, 633201. <utt> A: Oh, I'd better write it down, otherwise I'll probably forget it. <utt> B: I have already done it, Mr. Blank. It's on your desk. \n concepts in the answer: 

receive, phone, blank, office

9

answer: Miss grey received a phone call from david brown when mr blank was not in his office. \n corrupted concepts:  \n context: A: Any messages, Miss Grey? <utt> B: Just one, Mr. Blank. You had a telephone call from someone called Brown, David Brown. <utt> A: Brown? I don't seem to know anyone called Brown. What did he say? <utt> B: He wouldn't say. But it sounded important. I told him you'd phone him as soon as you got back. <utt> A: Well, I'd better do it then, I suppose. Er...you've got his phone number, haven't you? <utt> B: Yes, it's 633201. <utt> A: 622301. <utt> B: No, 633201. <utt> A: Oh, I'd better write it down, otherwise I'll probably forget it. <utt> B: I have already done it, Mr. Blank. It's on your desk. \n concepts in the target: 

telephone

10

Miss grey received a phone call from david brown when mr blank was not in his office. <utt> Miss grey gave the number to mr blank. <utt> David brown has an important work with mr blank. <utt> The listener tries to recall if he knows mr. brown personally. <utt> Mr blank is curious to know what message mr david has passed.

0 4 3 1 2

11

A: Brown? I don't seem to know anyone called Brown. What did he say? <utt> B: I have already done it, Mr. Blank. It's on your desk. <utt> A: Any messages, Miss Grey? <utt> A: 622301. <utt> B: No, 633201. <utt> B: Yes, it's 633201. <utt> A: Oh, I'd better write it down, otherwise I'll probably forget it. <utt> B: Just one, Mr. Blank. You had a telephone call from someone called Brown, David Brown. <utt> A: Well, I'd better do it then, I suppose. Er...you've got his phone number, haven't you? <utt> B: He wouldn't say. But it sounded important. I told him you'd phone him as soon as you got back.

2 9 0 6 7 5 8 1 4 3
